Higher order asymptotics for large deviations -- Part II

We obtain asymptotic expansions for the large deviation principle (LDP) for continuous time stochastic processes with weakly dependent increments. As a key example, we show that additive functionals of solutions of stochastic differential equations (SDEs) satisfying H\"ormander condition on a $d-$dimensional compact manifold admit these asymptotic expansions of all orders.

==> abbrev.tex <==

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}

%\newcommand{\fracinv}[2]{\frac{#2}{#1}}
%\newcommand{\eqdef}{\stackrel{\scriptscriptstyle\rm def}{=}}
%\newcommand{\lista}[2]{\text{${#1}$, $\ldots$, ${#2}$}}

%\def \proof{\medskip\noindent{\em Proof. }}
\def \qed{\hfill$\square$}

\def \mathEOPr{{\quad\rule{7pt}{7pt}}}
\def \Quad{{\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
\quad\quad\quad}}

\def \EOPr {{\rule{7pt}{7pt}\newline}}

\def\Dots{\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots
\dots\dots\dots\dots\dots\dots\dots\dots\dots\dots}

\def\ad{{\rm ad}}
\def\diam{{\rm diam}}
\def\dist{{\rm dist}}
\def\eps{{\varepsilon}}
\def\teps{{\tilde\varepsilon}}
\def\gr {{SL_d(\reals)}}
\def\length{{\rm length}}
\def\mes{{\rm mes}}
\def\supp{{\rm supp}}
\def\Area{{\rm Area}}
\def\Card{{\rm Card}}
\def\Const{{\rm Const}}
\def\Corr{{\rm Corr}}
\def\Cov{{\rm Cov}}
\def\Diff{{\rm Diff}}
\def\Div{{\rm div}}
\def\Int{{\rm Int}}
\def\Leb{{\rm Leb}}
\def\Lip{{\rm Lip}}
\def\Osc{\mathop{\rm Osc}}
\def\Prob{{\mathbb{P}}}
\def\tProb{{\tilde{\Prob}}}
\def\Tr{{\text{Tr}}}
\def\Var{{\rm Var}}
\def\Vol{{\rm Vol}}
\def\EXP{{\mathbb{E}}}
\def\tEXP{{\tilde\EXP}}
\def\PROJ{{\mathbb{P}}}
\def\SPR{{\mathbb{S}}}
\def\TOR{{\mathbb{T}}}

\def\vc{\omega*}

\def\fam{f_\varepsilon}

\def\BAN{\mathbb{B}}

\def\complex{\mathbb{C}}

\def\DDD{\mathbb{D}}

\def\bbI{\mathbb{I}}

\def\bbH{\mathbb{H}}

\def\bbP{\mathbb{P}}

\def\bbT{\mathbb{T}}

\def\bbX{\mathbb{X}}

\def\bbY{\mathbb{Y}}

\def\naturals{\mathbb{N}}

\def\Tor{\mathbb{T}}
\def\IS{\mathbb{S}}

\def\reals{\mathbb{R}}

\def\integers{\mathbb{Z}}



\def\RmII{{I\!\!I}}

\def\RmIII{{I\!\!I\!\!I}}

\def\RmIV{{I\!V}}


\def\P{{\partial }}



\def\TT {{\bf T}}



\def\UuEe{{\rm UuEe}}



\def\bA{\mathbf{A}}

\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}

\def\bD{\mathbf{D}}

\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bJ{\mathbf{J}}

\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}

\def\bM{\mathbf{M}}

\def\bN{\mathbf{N}}

\def\bO{\mathbf{O}}

\def\bP{\mathbf{P}}

\def\bQ{\mathbf{Q}}

\def\bR{\mathbf{R}}

\def\bS{\mathbf{S}}

\def\bT{\mathbf{T}}

\def\bV{\mathbf{V}}

\def\bX{\mathbf{X}}

\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\ba{\mathbf{a}}

\def\bb{\mathbf{b}}

\def\bc{\mathbf{c}}

\def\bd{\mathbf{d}}
\def\be{\mathbf{e}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
\def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bu{\mathbf{u}}
\def\bt{\mathbf{t}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\bz{\mathbf{z}}
\def\bkappa{\boldsymbol{\kappa}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bsigma{\boldsymbol{\sigma}}

\def\bPsi{{\boldsymbol{\Psi}}}

\def\tbq{\tilde{\mathbf{q}}}

\def\balpha{{\boldsymbol{\alpha}}}
\def\bphi{{\boldsymbol{\phi}}}
\def\btheta{{\boldsymbol{\theta}}}
\def\bomega{{\boldsymbol{\omega}}}

\def\bTheta{{\boldsymbol{\Theta}}}
\def\bDelta{{\boldsymbol{\Delta}}}

\def\btau{{\boldsymbol{\tau}}}

\def\bchi{{\boldsymbol{\chi}}}

\def\beps{{\boldsymbol{\varepsilon}}}



\def\brA{{\bar A}}

\def\brB{{\bar B}}

\def\brC{{\bar C}}

\def\brrC{{\bar\brC}}

\def\brD{{\bar D}}

\def\brbE{{\bar\bE}}

\def\brF{{\bar F}}

\def\brI{{\bar I}}

\def\brJ{{\bar J}}

\def\brrJ{{\bar{\brJ}}}

\def\brK{{\bar K}}

\def\brrK{{\bar\brK}}

\def\brL{{\bar L}}

\def\brM{{\bar M}}

\def\brN{{\bar N}}

\def\brP{{\bar P}}

\def\brbP{{\bar\bP}}

\def\brQ{{\bar Q}}

\def\brR{{\bar R}}

\def\brS{{\bar S}}

\def\brT{{\bar T}}

\def\brV{{\bar V}}

\def\brW{{\bar W}}

\def\brX{{\bar X}}

\def\brY{{\bar Y}}

\def\brcY{{\bar\cY}}

\def\brZ{{\bar Z}}

\def\bra{{\bar a}}

\def\brra{{\bar\bra}}

\def\brb{{\bar b}}

\def\brc{{\bar c}}

\def\brrc{{\bar \brc}}

\def\brbc{\mathbf{\brc}}

\def\brd{{\bar d}}

\def\brf{{\bar f}}

\def\brg{{\bar g}}

\def\brh{{\bar h}}

\def\brj{{\bar j}}

\def\brk{{\bar k}}

\def\brl{{\bar l}}

\def\brn{{\bar n}}

\def\brrn{{\bar{\bar n}}}

\def\brm{{\bar m}}

\def\brbm{{\bar \bm}}

\def\brq{{\bar q}}

\def\bru{{\bar{u}}}

\def\brbu{{\bar{u}}}

\def\brz{{\bar z}}

\def\brPsi{{\bar\Psi}}

\def\gammad{{\bar \gamma}}
\def\gammas{{\hat\gamma}}


\def\brp{{\bar p}}

\def\brrp{{\bar{\brp}}}

\def\brq{{\bar q}}

\def\brrq{{\bar{\brq}}}

\def\brs{{\bar s}}

\def\brt{{\bar t}}
\def\brrt{{\overline{\brt}}}

\def\brv{{\bar v}}

\def\brw{{\bar w}}

\def\brx{{\bar x}}

\def\brrx{{\bar{\brx}}}

\def\bry{{\bar y}}

\def\brDelta{{\bar \Delta}}

\def\brLambda{{\bar \Lambda}}

\def\bralpha{{\bar \alpha}}

\def\brbeta{{\bar \beta}}

\def\brdelta{{\bar \delta}}

\def\breps{{\bar\eps}}


\def\breta{{\bar \eta}}

\def\brreta{{\bar{\breta}}}

\def\brpi{{\bar \pi}}

\def\brgamma{{\bar \gamma}}

\def\brlambda{{\bar \lambda}}

\def\brnu{{\bar \nu}}

\def\brmu{{\bar \mu}}

\def\brxi{{\bar \xi}}

\def\brrho{{\bar\rho}}

\def\brtau{{\bar\tau}}

\def\brtheta{{\bar \theta}}

\def\brTheta{{\bar \Theta}}

\def\brsigma{{\bar \sigma}}

\def\brphi{{\bar \phi}}

\def\brPhi{{\bar \Phi}}

\def\brpsi{{\bar \psi}}

\def\brzeta{{\bar \zeta}}

\def\bromega{{\bar\omega}}

\def\brOmega{{\bar\Omega}}

\def\brbomega{{\bar\bomega}}

\def\brcG{{\bar{\cG}}}

\def\brcJ{{\bar{\cJ}}}

\def\bbM{{\mathbb{M}}}

\def\cA{\mathcal{A}}

\def\cB{\mathcal{B}}

\def\cb{\mathfrak{b}}

\def\cC{\mathcal{C}}

\def\cD{\mathcal{D}}

\def\cI{\mathcal{I}}

\def\cJ{\mathcal{J}}

\def\cF{\mathcal{F}}

\def\cG{\mathcal{G}}

\def\cH{\mathcal{H}}

\def\cE{\mathcal{E}}

\def\cK{\mathcal{K}}

\def\cL{\mathcal{L}}

\def\cM{\mathcal{M}}

\def\cN{\mathcal{N}}

\def\cO{\mathcal{O}}

\def\cP{\mathcal{P}}

\def\cQ{\mathcal{Q}}

\def\cR{\mathcal{R}}

\def\brcR{{\bar\cR}}

\def\cS{\mathcal{S}}

\def\cT{\mathcal{T}}

\def\cU{\mathcal{U}}

\def\cV{\mathcal{V}}

\def\cW{\mathcal{W}}

\def\cX{\mathcal{X}}

\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}


\def\dcD{{\partial\cD}}

\def\dcP{{\partial\cP}}

\def\DtK{{\tK^\diamond}}
\def\DcK{{\cK^\diamond}}
\def\DW{{W^\diamond}}


\def\fA{\mathfrak{A}}

\def\fB{\mathfrak{B}}

\def\fD{\mathfrak{D}}

\def\fF{\mathfrak{F}}

\def\fI{\mathfrak{I}}

\def\fJ{\mathfrak{J}}

\def\fK{\mathfrak{K}}

\def\fM{\mathfrak{M}}

\def\fN{\mathfrak{N}}

\def\fP{\mathfrak{P}}

\def\fQ{\mathfrak{Q}}

\def\fR{\mathfrak{R}}

\def\fS{\mathfrak{S}}

\def\fU{\mathfrak{U}}

\def\fX{\mathfrak{X}}

\def\fa{\mathfrak{a}}

\def\fb{\mathfrak{b}}

\def\fh{\mathfrak{h}}

\def\fn{\mathfrak{n}}

\def\ft{\mathfrak{t}}


\def\hA{{\hat A}}

\def\hcA{{\hat{\cA}}}

\def\hB{{\hat B}}

\def\hC{{\hat C}}

\def\hD{{\hat D}}

\def\hE{{\hat E}}

\def\hcE{{\hat{\cE}}}

\def\hF{{\hat F}}
\def\hcF{{\hat{\cF}}}

\def\hcG{{\hat\cG}}

\def\hH{{\hat H}}

\def\hI{{\hat I}}

\def\hJ{{\hat J}}

\def\hK{{\hat K}}

\def\hL{{\hat L}}

\def\hN{{\hat N}}

\def\hcM{{\hat{\cM}}}

\def\hP{{\hat P}}

\def\hQ{{\hat Q}}

\def\hbQ{{\hat{\bQ}}}

\def\hR{{\hat R}}

\def\hS{{\hat S}}

\def\hhS{{\hat \hS}}

\def\hcS{{\hat \cS}}

\def\hT{{\hat T}}

\def\phT{{\partial \hT}}

\def\hU{{\hat U}}

\def\hV{{\hat V}}

\def\hW{{\hat W}}

\def\hbV{{\hat{\bV}}}

\def\hX{{\hat X}}

\def\hY{{\hat Y}}

\def\hZ{{\hat Z}}

\def\ha{{\hat a}}

\def\hb{{\hat b}}

\def\hc{{\hat c}}

\def\hhc{{\hat \hc}}

\def\hd{{\hat d}}

\def\hf{{\hat f}}

\def\hg{{\hat g}}

\def\hh{{\hat h}}

\def\hl{{\hat l}}

\def\hm{{\hat m}}

\def\hn{{\hat n}}

\def\hht{{\hat t}}

\def\hp{{\hat p}}

\def\hq{{\hat q}}

\def\hs{{\hat s}}

\def\hu{{\hat u}}


\def\halpha{{\hat\alpha}}

\def\hbeta{{\hat\beta}}

\def\hgamma{{\hat\gamma}}

\def\hGamma{{\hat\Gamma}}

\def\hdelta{{\hat\delta}}

\def\heps{{\hat{\eps}}}

\def\hkappa{{\hat\kappa}}

\def\hLambda{{\hat\Lambda}}

\def\hmu{{\hat\mu}}

\def\hnu{{\hat\nu}}

\def\hchi{{\hat\chi}}

\def\hxi{{\hat\xi}}

\def\hrho{{\hat\rho}}

\def\hsigma{{\hat\sigma}}

\def\heta{{\hat\eta}}

\def\hpsi{{\hat\psi}}

\def\htheta{{\hat\theta}}

\def\hbtheta{{\hat\btheta}}

\def\hTheta{{\hat\Theta}}

\def\hzeta{{\hat\zeta}}

\def\hOmega{{\hat\Omega}}

\def\hbomega{{\hat\bomega}}

\def\hDelta{\hat{\mathbf{\Delta}}}


\def\llambda{\underline{\lambda}}

\def\lchi{\underline{\chi}}



\def\sA{\EuScript{A}}

\def\sB{\EuScript{B}}

\def\sD{\EuScript{D}}

\def\sE{\EuScript{E}}

\def\sG{\EuScript{G}}

\def\sH{\EuScript{H}}

\def\sL{\EuScript{L}}

\def\sM{\EuScript{M}}

\def\sF{\EuScript{F}}

\def\sX{\EuScript{X}}

\def\sU{\EuScript{U}}

\def\sV{\EuScript{V}}

\def\sW{\EuScript{W}}





\def\tA{{\tilde A}}

\def\tcA{{\tilde \cA}}

\def\ttcA{{\tilde{\tilde{\mathcal{A}}}}}

\def\tB{{\tilde B}}

\def\tC{{\tilde C}}

\def\tD{{\tilde D}}

\def\ttD{{\tilde \tD}}

\def\tE{{\tilde E}}

\def\tF{{\tilde F}}

\def\tcD{{\tilde \cD}}
\def\tcF{{\tilde \cF}}
\def\tcG{{\tilde \cG}}

\def\ttcG{{\tilde {\tilde\cG}}}

\def\tH{{\tilde H}}

\def\ttH{{\tilde \tH}}

\def\tI{{\tilde I}}

\def\tcI{{\tilde\cI}}

\def\tK{{\tilde K}}

\def\tL{{\tilde L}}

\def\tcM{{\tilde\cM}}

\def\tP{{\tilde P}}

\def\tR{{\tilde R}}

\def\tQ{{\tilde Q}}

\def\tS{{\tilde S}}

\def\ttS{{\tilde\tS}}

\def\tcS{{\tilde \cS}}

\def\tT{{\tilde T}}

\def\tX{{\tilde X}}

\def\tV{{\tilde V}}

\def\tW{{\tilde W}}

\def\tcX{{\tilde \cX}}

\def\tY{{\tilde Y}}

\def\tZ{{\tilde Z}}

\def\ta{{\tilde a}}

\def\tta{{\tilde{\ta}}}

\def\tb{{\tilde b}}

\def\ttb{{\tilde{\tb}}}

\def\tc{{\tilde c}}

\def\ttc{{\tilde \tc}}

\def\tf{{\tilde f}}

\def\tg{{\tilde g}}

\def\th{{\tilde h}}

\def\tj{{\tilde j}}

\def\ttj{{\tilde\tj}}

\def\tth{{\tilde{\th}}}

\def\tk{{\tilde k}}

\def\tl{{\tilde l}}

\def\tm{{\tilde m}}

\def\ttm{{\tilde{\tilde m}}}

\def\tn{{\tilde n}}

\def\ttn{{\tilde \tn}}

\def\tp{{\tilde p}}

\def\ttp{{\tilde \tp}}

\def\tr{{\tilde r}}

\def\ts{{\tilde s}}

\def\tts{{\tilde{\tilde s}}}

\def\Tt{{\tilde{t}}}

\def\TTt{{\tilde{\Tt}}}

\def\tu{{\tilde u}}

\def\ttt{{\tilde t}}

\def\tv{{\tilde v}}

\def\tw{{\tilde w}}

\def\tx{{\tilde x}}

\def\ttx{{\tilde{\tilde x}}}

\def\ty{{\tilde y}}

\def\tz{{\tilde z}}

\def\talpha{{\tilde\alpha}}

\def\tbeta{{\tilde\beta}}

\def\tgamma{{\tilde\gamma}}

\def\ttgamma{{\tilde{\tilde{\gamma}}}}

\def\tdelta{{\tilde\delta}}
\def\tDelta{{\tilde{\mathbf{\Delta}}}}

\def\teps{{\tilde\varepsilon}}

\def\tkappa{{\tilde\kappa}}

\def\tlambda{{\tilde\lambda}}

\def\tmu{{\tilde\mu}}

\def\tnu{{\tilde\nu}}

\def\teta{{\tilde\eta}}

\def\tpi{{\tilde\pi}}

\def\trho{{\tilde\rho}}

\def\ttrho{{\tilde{\tilde\rho}}}

\def\tphi{{\tilde\phi}}

\def\tPsi{{\tilde\Psi}}

\def\tsigma{{\tilde\sigma}}

\def\ttheta{{\tilde\theta}}

\def\tTheta{{\tilde\Theta}}

\def\tzeta{{\tilde\zeta}}

\def\tchi{{\tilde\chi}}

\def\txi{{\tilde\xi}}

\def\tomega{{\tilde{\omega}}}

\def\tGamma{{\tilde{\Gamma}}}

\def\tPhi{{\tilde{\Phi}}}
\def\ttPhi{{\tilde{\tPhi}}}

\def\tOmega{{\tilde{\Omega}}}

\def\tcB{{\tilde{\mathcal{B}}}}

\def\tcR{\tilde{\mathcal{R}}}

\def\tPi{{\tilde \Pi}}

\def\ttPi{{\tilde{\tilde{\Pi}}}}

\def\ttu{{\tilde{\tilde{u}}}}

\def\tell{{\tilde\ell}}
\def\ttell{{\tilde{\tilde\ell}}}

\def\unp{{\underline{p}}}

%\makeatletter

%\renewcommand{\section}{\@startsection {section}{1}{\z@}%
 %                                  {-3.5ex \@plus -1ex \@minus -.2ex}%
 %                                  {2.3ex \@plus.2ex}%
  %                                 {\normalfont\large\bfseries}}
%\renewcommand{\subsection}[1]{\@startsection{subsection}{2}{\z@}%
%   {-2.5ex\@plus -1ex \@minus -.2ex}%
%    {-.0em}
%    {\reset@font\bfseries}{#1}{\bf .}}
\makeatother

\def\la{\langle}
\def\ra{\rangle}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

